Grounded Human-Object Interaction Hotspots from Video (Extended Abstract)

Learning how to interact with objects is an important step towards embodied visual intelligence, but existing techniques suffer from heavy supervision or sensing requirements. We propose an approach to learn human-object interaction "hotspots" directly from video. Rather than treat affordances as a manually supervised semantic segmentation task, our approach learns about interactions by watching videos of real human behavior and anticipating afforded actions. Given a novel image or video, our model infers a spatial hotspot map indicating how an object would be manipulated in a potential interaction, even if the object is currently at rest. Through results with both first and third person video, we show the value of grounding affordances in real human-object interactions. Not only are our weakly supervised hotspots competitive with strongly supervised affordance methods, but they can also anticipate object interaction for novel object categories. Project page: http://vision.cs.utexas.edu/projects/interaction-hotspots/

==> sections/related.tex <==
\section{Related Work}

\vspace{0.05in}
\noindent\textbf{Visual Affordances}.
The theory of affordances \cite{gibson1979ecological}, originally from work in psychology, has been adopted to study several tasks in computer vision~\cite{hassanin2018visual}. 
In action understanding, affordances provide context for action anticipation~\cite{koppula2016anticipating,rhinehart2016learning,zhou2016cascaded} and  help learn stronger action recognition models~\cite{koppula2013learning}.
In scene understanding, they help decide \textit{where} in a scene a particular action can be performed \cite{savva2014scenegrok,grabner2011makes,wang2017binge,delaitre2012scene}, learn scene geometry~\cite{gupta20113d,fouhey2014people}, or understand social situations~\cite{chuang2017learning}.
In object understanding, affordances help model object function and interaction~\cite{stark2008functional,yao2010grouplet,zhu2015understanding}, and have been studied jointly with hand pose/configuration~\cite{kjellstrom2011visual,thermos2017deep,castellini2011using} and object motion~\cite{gupta2007objects,gupta2009observing}. %

The choice of affordance representation varies significantly in these tasks, spanning across human pose, trajectories of objects, sensorimotor grasps, and 3D scene reconstructions. Often, this results in specialized hardware and heavy sensor requirements (\eg, force gloves, depth cameras). We propose to %
automatically learn appropriate representations for visual affordances  directly from RGB video of human-object interactions.
%


\vspace{0.05in}
\noindent\textbf{Grounded Affordances}.
Pixel-level segmentation of object parts~\cite{sawatzky2017weakly,myers2015affordance,nguyen2017object} is a common affordance representation, for which 
supervised semantic segmentation frameworks are the typical %
approach~\cite{myers2015affordance,roy2016multi,nguyen2017object,do2017affordancenet}. These segmentations convey high-level information about object function, but rely on manual mask annotations to train---which are not only costly, but can also give an unrealistic view of how objects are actually used.  Unlike our approach, such methods are ``ungrounded" in the sense that the annotator declares regions of interest on the objects outside of any interaction context.
%

Representations that are grounded in human behavior have also been explored. In images, human body pose serves as a proxy for object affordance to reveal 
modes of interaction with musical instruments~\cite{yao2010grouplet,yao2013discovering} or likely object interaction regions~\cite{chaoyeh-ijcv2016}.  
Given a video, methods can parse 3D models 
to estimate physical concepts (velocity, force, etc.) in order to categorize object interactions~\cite{zhu2016inferring,zhu2015understanding}.  For instructional video, methods explore ways to extract object states~\cite{alayrac2017joint}, modes of object interaction~\cite{damen2014you}, interaction regions~\cite{fang2018demo2vec}, or the anticipated trajectory of an object given a person's skeleton pose~\cite{koppula2014physically}. %
%

We introduce a new approach for learning affordance ``heatmaps" grounded in human-object interaction, as
%
derived directly from watching real-world videos of people using the objects.
Our model differs from other approaches in two main ways. First, no prior about interaction in the form of human pose, hand position, or 3D object reconstruction is used. All information about the interactions is learned directly from video. Second, %
rather than learn from manually annotated ground truth masks or keypoints~\cite{myers2015affordance,roy2016multi,nguyen2017object,do2017affordancenet,sawatzky2017weakly,sawatzky2017adaptive,fang2018demo2vec}, 
our model uses only coarse action labels for video clips to guide learning.

%
%


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%

\vspace{0.05in}
\noindent\textbf{Video anticipation}. 
Predicting future frames in videos has been studied extensively in computer vision~\cite{ranzato2014video,mathieu2015deep,vondrick2017generating,liang2017dual,srivastava2015unsupervised,villegas2017learning,walker2017pose,oh2015action,xue2016visual,vondrick2016generating,jayaraman2018time}. Future prediction has been applied to action anticipation~\cite{huang2014action,vondrick2015anticipating,koppula2016anticipating,rhinehart2018forecast}, active-object forecasting~\cite{furnari2017next}, %
%
and to guide demonstration learning in robotics~\cite{finn2016unsupervised,finn2017deep,ebert2017self}.
%
In contrast to these works, we 
%
devise a novel anticipation task---learning object interaction affordances from video. 
%
Rather than predict future frames or action labels, our model anticipates 
%
correspondences between \emph{inactive} objects (at rest, and not interacted with) and \emph{active} objects (undergoing interaction) in feature space, which we then use to estimate affordances.

